On the Simulation Power of Surface Chemical Reaction Networks

The Chemical Reaction Network (CRN) is a well-studied model that describes the interaction of molecules in well-mixed solutions. In 2014, Qian and Winfree [22] proposed the abstract surface chemical reaction network model (sCRN), which takes the advantage of spatial separation by placing molecules on a structured surface, limiting the interaction between molecules. In this model, molecules can only react with their immediate neighbors. Many follow up works study the computational and pattern-construction power of sCRNs. In this work, our goal is to describe the power of sCRN by relating the model to other well-studied models in distributed computation. In this work, our main result is to show that, given the same initial configuration, sCRN, affinity strengthening tile automata, cellular automata, and amoebot can all simulate each other (up to unavoidable rotation and reflection of the pattern). One of our techniques is a coloring on-the-fly, which allows all molecules in sCRN to have a global orientation.

==> ref.tex <==
QW14:
explain an abstract model of CRN on a surface, propose a theoretical framework that uses a novel DNA strand displacement mechanism to implement abstract chemical reaction networks (CRNs) on the surface of a DNA nanostructure, and show that sCRN can perform efficient alg computation and create complex spatial dynamics.
systematic approaches for building continually active logic circuits and cellular automata.

CQW20:
Emulate asynchronous/synchronous CA, implement continuously active boolean logic circuits. Manufacture complex spatial patterns from simple initial conditions.
trade-off between the ability of precisely place molecules and precisely control molecular interactions.
several open problems.

AB23:
complexity of reconfiguration problem (whether a given configuration can ever transform into another configuration)

RW00:
Tile assembly model, consider single seed system. 
$O(\log N)$ complexity (minimum number of distinct tiles required) that self-assemble a $N\times N$ square under temperature $\tau=2$.

AGH03:
use Tile assembly model defined above, opt complexity (meet Kolmogorov complexity) $\theta(\frac{\log n}{\log\log n})$ complexity for $n\time n$ square by considering a base-$b$ counter.

HP23:
simulation definition. Simulation between model variations of aTAM.
mapping is a partial function from $m$-block macrotile to a tile.
''fuzz'': non-empty block $\alpha'$ satisfies $(x,y,z)+(u_x,u_y,u_z)\in$ domain $\alpha$. $\norm{(u_x,u_y,u_z)}\leq1$: map cleanly.

GOT15:
freezing CA definition

ka05:
synchronous cellular automata survey.

BNR20:
survey on cellular automata, sync/async

Na20:
survey on async CA (1d)

GMM21:
decide if there exists a seq of updating acheme that changes the state of a given cell.

CL18:
freezing TA model, simulation definition, c-fuzz: $(x,y)+(u,v)\in$ domain. $\maxnorm{(u,v)}\leq c$.

CGS21:
complexity of Unique assembly verification problem (if a given system uniquely produce an assembly) with different restriction (freezing, affinity strengthening)

ADD19:
TA simulate ameobot, simulation definition

RDS23:
unit seed TA definition, corollary?

DDG14:
ameobot model

